CALYPSO: LLMs as Dungeon Masters' Assistants

The role of a Dungeon Master, or DM, in the game Dungeons & Dragons is to perform multiple tasks simultaneously. The DM must digest information about the game setting and monsters, synthesize scenes to present to other players, and respond to the players' interactions with the scene. Doing all of these tasks while maintaining consistency within the narrative and story world is no small feat of human cognition, making the task tiring and unapproachable to new players. Large language models (LLMs) like GPT-3 and ChatGPT have shown remarkable abilities to generate coherent natural language text. In this paper, we conduct a formative evaluation with DMs to establish the use cases of LLMs in D&D and tabletop gaming generally. We introduce CALYPSO, a system of LLM-powered interfaces that support DMs with information and inspiration specific to their own scenario. CALYPSO distills game context into bite-sized prose and helps brainstorm ideas without distracting the DM from the game. When given access to CALYPSO, DMs reported that it generated high-fidelity text suitable for direct presentation to players, and low-fidelity ideas that the DM could develop further while maintaining their creative agency. We see CALYPSO as exemplifying a paradigm of AI-augmented tools that provide synchronous creative assistance within established game worlds, and tabletop gaming more broadly.

==> utils.tex <==
\usepackage{xcolor}
\usepackage{xifthen}
\newcommand\todo[1]{
    \textcolor{red}{
        \ifthenelse{\isempty{#1}}
            {TODO}
            {TODO: #1}
    }
}

\newcommand{\dagsuper}[0]{\textsuperscript{\textdagger}}
\newcommand{\starsuper}[0]{\textsuperscript{*}}

\newcommand\zhu[1]{\textcolor{blue}{#1}}

\newcommand\lara[1]{\textcolor{purple}{Lara: #1}}
